Prioritise the Best Variation

Binary session types guarantee communication safety and session fidelity, but alone they cannot rule out deadlocks arising from the interleaving of different sessions. In Classical Processes (CP)$-$a process calculus based on classical linear logic$-$deadlock freedom is guaranteed by combining channel creation and parallel composition under the same logical cut rule. Similarly, in Good Variation (GV)$-$a linear concurrent $\lambda$-calculus$-$deadlock freedom is guaranteed by combining channel creation and thread spawning under the same operation, called fork. In both CP and GV, deadlock freedom is achieved at the expense of expressivity, as the only processes allowed are tree-structured. Dardha and Gay define Priority CP (PCP), which allows cyclic-structured processes and restores deadlock freedom by using priorities, in line with Kobayashi and Padovani. Following PCP, we present Priority GV (PGV), a variant of GV which decouples channel creation from thread spawning. Consequently, we type cyclic-structured processes and restore deadlock freedom by using priorities. We show that our type system is sound by proving subject reduction and progress. We define an encoding from PCP to PGV and prove that the encoding preserves typing and is sound and complete with respect to the operational semantics.

==> fig/pgv-scheduler.tex <==
\begin{figure}
  \centering
  \begin{tikzpicture}
    \node[shape=circle,draw=black]                       (agent1) {\tm{\agent1}};
    \node[shape=circle,draw=black,below right=of agent1] (agent2) {\tm{\agent2}};
    \node[shape=circle,draw=black,below left =of agent1] (agent3) {\tm{\agent3}};

    \node[shape=circle,draw=black,above      =of agent1] (proc1) {\tm{\proc1}};
    \node[shape=circle,draw=black,below right=of agent2] (proc2) {\tm{\proc2}};
    \node[shape=circle,draw=black,below left =of agent3] (proc3) {\tm{\proc3}};

    \draw[->]
    (agent1) -- node[pos=0.35,above] {$c_1$}
    node[pos=1.0,above] {$c'_1$} ++ (agent2);
    \draw[->]
    (agent2) -- node[pos=0.1,above] {$c_2$}
    node[pos=0.9,above] {$c'_2$} ++ (agent3);
    \draw[->]
    (agent3) -- node[pos=0.0,above] {$c_3$}
    node[pos=0.65,above] {$c'_3$} ++ (agent1);
       
    \draw[implies-implies,double]
    (agent1) -- node[pos=0.15,left] {$a_1$} node[pos=0.85,left] {$a'_1$}
    node[pos=0.15,right] {$b_1$} node[pos=0.85,right] {$b'_1$} ++ (proc1);
    \draw[implies-implies,double]
    (agent2) -- node[pos=0.15,above right] {$a_2$} node[pos=0.85,above right] {$a'_2$}
    node[pos=0.15,below left] {$b_2$} node[pos=0.85,below left] {$b'_2$} ++ (proc2);
    \draw[implies-implies,double]
    (agent3) -- node[pos=0.15,above left] {$a_3$} node[pos=0.85,above left] {$a'_3$}
    node[pos=0.15,below right] {$b_3$} node[pos=0.85,below right] {$b'_3$} ++ (proc3);

    \draw[->]
    (agent1) to[bend left=45] node[pos=0.15,left] {$d$} node[pos=0.85,left] {$d'$} (proc1);

    \draw[->,dashed]
    (proc1.east) to[bend left] node[pos=0.15,align=center,above right] {optional\\data transfer} (proc2.north);
    \draw[->,dashed]
    (proc2.west) to[bend left] (proc3.east);
    \draw[->,dashed]
    (proc3.north) to[bend left] (proc1.west);
  \end{tikzpicture}
  \label{fig:pgv-scheduler}
  \caption{Milner's Cyclic Scheduler}
\end{figure}

%%% Local Variables:
%%% TeX-master: "../priorities"
%%% End:


==> priority-cp.tex <==
\section{Relation to Priority CP}\label{sec:pcp}

We present a correspondence between Priority GV and an updated version of Priority CP~\cite[PCP]{dardhagay18extended}, which is Wadler's CP~\cite{wadler14} with priorities. This correspondence connects PGV to (a~relaxed variant of) classical linear logic.

\subsection{Revisiting Priority CP}
\begingroup
\usingnamespace{pcp}
\textbf{Types} ($\ty{A}$, $\ty{B}$) in PCP correspond to linear logic connectives annotated with priorities $\cs{o}\in\mathbb{N}$. Typing environments, duality, and the priority function $\pr(\cdot)$ are defined as expected.
\[
  \begin{array}{lcl}
    \ty{A}, \ty{B}
     & \Coloneqq & \ty{\tytens[\cs{o}]{A}{B}}
    \sep        \ty{\typarr[\cs{o}]{A}{B}}
    \sep        \ty{\tyone[\cs{o}]}
    \sep        \ty{\tybot[\cs{o}]}
    \sep        \ty{\typlus[\cs{o}]{A}{B}}
    \sep        \ty{\tywith[\cs{o}]{A}{B}}
    \sep        \ty{\tynil[\cs{o}]}
    \sep        \ty{\tytop[\cs{o}]}
  \end{array}
\]
\textbf{Processes} ($\tm{P}$, $\tm{Q}$) in PCP are defined by the following grammar.
\[
  \begin{array}[t]{lcl}
    \tm{P}, \tm{Q}
     & \Coloneqq & \tm{\link{x}{y}}
    \sep   \tm{\res{x}{y}{P}}
    \sep   \tm{(\ppar{P}{Q})}
    \sep   \tm{\halt}
    \\   & \sep & \tm{\send{x}{y}{P}}
    \sep   \tm{\close{x}{P}}
    \sep   \tm{\recv{x}{y}{P}}
    \sep   \tm{\wait{x}{P}}
    \\   & \sep & \tm{\inl{x}{P}}
    \sep   \tm{\inr{x}{P}}
    \sep   \tm{\offer{x}{P}{Q}}
    \sep   \tm{\absurd{x}}
  \end{array}
\]
Processes are typed by sequents $\seq{P}{\ty{\Gamma}}$, which correspond to the one-sided sequents in classical linear logic. Differently from PGV, in PCP we do not need to store the greatest priority on the sequent, as, due to the absence of higher-order functions, we cannot compose processes \emph{sequentially}.

PCP decomposes cut into \LabTirName{T-Res} and \LabTirName{T-Par} rules---corresponding to cycle and mix rules, respectively---and guarantees deadlock freedom by using priority constraints, \eg, as in \LabTirName{T-Send}.
\begin{mathpar}
  \small
  \inferrule*[lab=T-Res]{
    \seq{P}{\ty{\Gamma},\tmty{x}{A},\tmty{y}{\co{A}}}
  }{\seq{\res{x}{y}{P}}{\ty{\Gamma}}}
  \inferrule*[lab=T-Par]{
    \seq{P}{\ty{\Gamma}}
    \and
    \seq{Q}{\ty{\Delta}}
  }{\seq{\ppar{P}{Q}}{\ty{\Gamma},\ty{\Delta}}}
  \inferrule*[lab=T-Send]{
    \seq{P}{\ty{\Gamma},\tmty{y}{A},\tmty{x}{B}}
    \and
    \cs{o}<\minpr(\ty{\Gamma},\ty{A},\ty{B})
  }{\seq{\send{x}{y}{P}}{\ty{\Gamma},\tmty{x}{\tytens[\cs{o}]{A}{B}}}}
\end{mathpar}

The main change we make to PCP is \emph{removing commuting conversions} and defining an operational semantics based on structural congruence. Commuting conversions are necessary if we want our reduction strategy to correspond \emph{exactly} to cut elimination.
However, from the perspective of process calculi, commuting conversions behave strangely: they allow an input/output action to be moved to the top of a process, thus potentially blocking actions which were previously possible. This makes CP, and Dardha and Gay's PCP~\cite{dardhagay18extended}, non-confluent.
As Lindley and Morris~\cite{lindleymorris15} show, all communications that can be performed \emph{with} the use of commuting conversions, can also be performed \emph{without} them, using structural congruence.

%Consider the commuting conversion $(\kappa_{\parr})$ for $\pcp{\tm{\recv{x}{y}{P}}}$:
%\begin{mathpar}
%  (\kappa_{\parr})
%  \quad
%  \tm{\res{z}{z'}{(\ppar{\recv{x}{y}{P}}{Q})}}
%  \red
%  \tm{\recv{x}{y}{\res{z}{z'}{(\ppar{P}{Q})}}}
%\end{mathpar}
%As a result of $(\kappa_{\parr})$, $\pcp{\tm{Q}}$ becomes blocked on $\pcp{\tm{\labrecv{x}{y}}}$, and any actions $\pcp{\tm{Q}}$ was able to perform become unavailable. Consequently, CP is non-confluent:
%\begin{mathpar}
%  \setlength{\arraycolsep}{2em}
%  \begin{array}{cc}
%    \multicolumn{2}{c}{%
%    \hspace*{10ex}
%    {\tm{\res{x}{x'}{(\ppar{\recv{a}{y}{P}}{\res{z}{z'}{(\ppar{\close{z}{\halt}}{\wait{z'}{Q}})}})}}}}
%    \\
%    \qquad\rotatebox[origin=c]{270}{$\red\hphantom{{}^+}$}
%    &
%    \rotatebox[origin=c]{270}{$\red^+$}\qquad
%    \\
%    {\tm{\recv{a}{y}{\res{x}{x'}{(\ppar{P}{\res{z}{z'}{(\ppar{\close{z}{\halt}}{\wait{z'}{Q}})}})}}}}
%    &
%    {\tm{\recv{a}{y}{\res{x}{x'}{(\ppar{P}{Q})}}}}
%  \end{array}
%\end{mathpar}

In  particular for PCP, commuting conversions break our intuition that an action with lower priority \emph{occurs before} an action with higher priority. To cite Dardha and Gay~\cite{dardhagay18extended} ``\emph{if a prefix on a channel endpoint $\pcp{\tm{x}}$ with priority $\cs{o}$ is pulled out at top level, then to preserve priority constraints in the typing rules [..], it is necessary to increase priorities of all actions after the prefix on $\pcp{\tm{x}}$}'' by $\cs{o+1}$.
One benefit of removing commuting conversions is that we no longer need to dynamically change the priorities during reduction, which means that the intuition for priorities holds true in our updated version of PCP. Furthermore, we can safely define reduction on untyped processes, which means that type and priority information is erasable!

We prove closed progress for our updated PCP.
\begin{thm}\label{thm:pcp-closed-progress}
  %[Progress, $\pcp{\red}$]%
  If $\pcp{\seq{P}{\emptyenv}}$, then either $\pcp{\tm{P}=\tm{\halt}}$ or there exists a $\pcp{\tm{Q}}$ such that $\pcp{\tm{P}\red\tm{Q}}$.
\end{thm}
\endgroup

\subsection{Correspondence between PGV and PCP}
\begingroup
We illustrate the relation between PCP and PGV by defining a translation from PCP to PGV. The translation on types is defined as follows:
\[
  \begin{array}{lcl}
    \ty{\cpgvT{\pcp{\tytens[\cs{o}]{A}{B}}}}
     & = & \pgv{\ty{\tysend[\cs{o}]{\co{\cpgvT{A}}}{\cpgvT{B}}}}
    \\
    \ty{\cpgvT{\pcp{\typlus[\cs{o}]{A}{B}}}}
     & = & \pgv{\ty{\tyselect[\cs{o}]{\cpgvT{A}}{\cpgvT{B}}}}
  \end{array}
  \;
  \begin{array}{lcl}
    \ty{\cpgvT{\pcp{\tyone[\cs{o}]}}}
     & = & \ty{\pgv{\tyends[\cs{o}]}}
    \\
    \ty{\cpgvT{\pcp{\tynil[\cs{o}]}}}
     & = & \pgv{\ty{\tyselectemp[\cs{o}]}}
  \end{array}
  \;
  \begin{array}{lcl}
    \ty{\cpgvT{\pcp{\typarr[\cs{o}]{A}{B}}}}
     & = & \pgv{\ty{\tyrecv[\cs{o}]{\cpgvT{A}}{\cpgvT{B}}}}
    \\
    \ty{\cpgvT{\pcp{\tywith[\cs{o}]{A}{B}}}}
     & = & \pgv{\ty{\tyoffer[\cs{o}]{\cpgvT{A}}{\cpgvT{B}}}}
  \end{array}
  \;
  \begin{array}{lcl}
    \ty{\cpgvT{\pcp{\tybot[\cs{o}]}}}
     & = & \ty{\pgv{\tyendr[\cs{o}]}}
    \\
    \ty{\cpgvT{\pcp{\tytop[\cs{o}]}}}
     & = & \pgv{\ty{\tyofferemp[\cs{o}]}}
  \end{array}
\]

There are two separate translations on processes. The main translation, $\tm{\cpgvM{\cdot}}$, translates processes to \emph{terms}:
\begin{align*}
   & \pcp{\tm{\cpgvM{\link{x}{y}}}}
   &                                    & = \pgv{\tm{\link\;{\pair{x}{y}}}}                                               \\
   & \pcp{\tm{\cpgvM{\res{x}{y}{P}}}}
   &                                    & = \pgv{\tm{\letpair{x}{y}{\new}{\cpgvM{P}}}}                                    \\
   & \pcp{\tm{\cpgvM{\ppar{P}{Q}}}}
   &                                    & = \pgv{\tm{\andthen{\spawn\;{(\lambda\unit.\cpgvM{P})}}{\cpgvM{Q}}}}            \\
   & \pcp{\tm{\cpgvM{\halt}}}
   &                                    & = \pgv{\tm{\unit}}                                                              \\
   & \pcp{\tm{\cpgvM{\close{x}{P}}}}
   &                                    & = \pgv{\tm{\andthen{\close\;{x}}{\cpgvM{P}}}}                                   \\
   & \pcp{\tm{\cpgvM{\wait{x}{P}}}}
   &                                    & = \pgv{\tm{\andthen{\wait\;{x}}{\cpgvM{P}}}}                                    \\
   & \pcp{\tm{\cpgvM{\send{x}{y}{P}}}}
   &                                    & = \pgv{\tm{\letpair{y}{z}{\new}{\letbind{x}{\send\;{\pair{z}{x}}}{\cpgvM{P}}}}} \\
   & \pcp{\tm{\cpgvM{\recv{x}{y}{P}}}}
   &                                    & = \pgv{\tm{\letpair{y}{x}{\recv\;{x}}{\cpgvM{P}}}}                              \\
   & \pcp{\tm{\cpgvM{\inl{x}{P}}}}
   &                                    & = \pgv{\tm{\letbind{x}{\select{\labinl}\;{x}}{\cpgvM{P}}}}                      \\
   & \pcp{\tm{\cpgvM{\inr{x}{P}}}}
   &                                    & = \pgv{\tm{\letbind{x}{\select{\labinr}\;{x}}{\cpgvM{P}}}}                      \\
   & \pcp{\tm{\cpgvM{\offer{x}{P}{Q}}}}
   &                                    & = \pgv{\tm{\offer{x}{x}{\cpgvM{P}}{x}{\cpgvM{Q}}}}                              \\
   & \pcp{\tm{\cpgvM{\absurd{x}}}}
   &                                    & = \pgv{\tm{\offeremp{x}}}
\end{align*}

Unfortunately, the operational correspondence along $\tm{\cpgvM{\cdot}}$ is unsound, as it translates $\nu$-binders and parallel compositions to $\pgv{\tm{\new}}$ and $\pgv{\tm{\spawn}}$, which can reduce to their equivalent configuration constructs using \LabTirName{E-New} and \LabTirName{E-Spawn}. The same goes for $\nu$-binders which are inserted when translating bound send to unbound send. For instance, the process $\pcp{\tm{\send{x}{y}{P}}}$ is blocked, but its translation uses $\pgv{\tm{\new}}$ and can reduce. To address this issue, we use a second translation, $\tm{\cpgvC{\cdot}}$, which is equivalent to $\tm{\cpgvM{\cdot}}$ followed by reductions using \LabTirName{E-New} and \LabTirName{E-Spawn}:
\begin{align*}
   & \pcp{\tm{\cpgvC{\res{x}{y}{P}}}}
   &                                   & = \pgv{\tm{\res{x}{y}{\cpgvC{P}}}}
  \\
   & \pcp{\tm{\cpgvC{\ppar{P}{Q}}}}
   &                                   & = \pgv{\tm{\ppar{\cpgvC{P}}{\cpgvC{Q}}}}
  \\
   & \pcp{\tm{\cpgvC{\send{x}{y}{P}}}}
   &                                   & = \pgv{\tm{\res{y}{z}{(\child\;\letbind{x}{\send\;\pair{z}{x}}{\cpgvM{P}})}}}
  \\
   & \pcp{\tm{\cpgvC{\inl{x}{P}}}}
   &                                   & = \pgv{\tm{\res{y}{z}{(\child\;\letbind{x}{\andthen{\close\;(\send\;\pair{\inl{y}}{x})}{z}}{\cpgvM{P}})}}}
  \\
   & \pcp{\tm{\cpgvC{\inr{x}{P}}}}
   &                                   & = \pgv{\tm{\res{y}{z}{(\child\;\letbind{x}{\andthen{\close\;(\send\;\pair{\inr{y}}{x})}{z}}{\cpgvM{P}})}}}
  \\
   & \pcp{\tm{\cpgvC{P}}}
   &                                   & = \pgv{\tm{\child{\cpgvM{P}}}},\quad\text{if none of the above apply}
\end{align*}

Typing environments are translated pointwise, and sequents $\pcp{\seq{P}{\ty{\Gamma}}}$ are translated as $\pgv{\cseq[\child]{\ty{\cpgvT{\ty{\Gamma}}}}{\cpgvC{P}}}$, where $\tm{\pgv{\child}}$ indicates a child thread. Translated processes do not have a main thread.
The translations $\tm{\cpgvM{\cdot}}$ and $\tm{\cpgvC{\cdot}}$ preserve typing, and the latter induces a sound and complete operational correspondence.
\begin{lem}\label{lem:pcp-to-pgv-terms-preservation}
  %[Preservation, ${\tm{\cpgvM{\cdot}}}$]%
  If $\pcp{\seq{P}{\ty{\Gamma}}}$, then $\pgv{\tseq[\cs{p}]{\ty{\cpgvT{\Gamma}}}{\cpgvM{P}}{\tyunit}}$.
\end{lem}
\begin{thm}\label{thm:pcp-to-pgv-confs-preservation}
  %[Preservation, ${\tm{\cpgvC{\cdot}}}$]%
  If $\pcp{\seq{P}{\ty{\Gamma}}}$, then $\pgv{\cseq[\child]{\ty{\cpgvT{\Gamma}}}{\cpgvC{P}}}$.
\end{thm}
\begin{lem}\label{lem:pcp-to-pgv-cpgvM-to-cpgvC}
  For any $\pcp{\tm{P}}$, either:
  \begin{itemize}
    \item $\pgv{\tm{\child\;\cpgvM{P}}=\tm{\cpgvC{P}}}$; or
    \item $\pgv{\tm{\child\;\cpgvM{P}}\cred^+\tm{\cpgvC{P}}}$, and for any $\pgv{\tm{\conf{C}}}$, if $\pgv{\tm{\child\;\cpgvM{P}}\cred\tm{\conf{C}}}$, then $\pgv{\tm{\conf{C}}\cred^\star\tm{\cpgvC{P}}}$.
  \end{itemize}
\end{lem}
\begin{thm}\label{thm:pcp-to-pgv-operational-correspondence-soundness}
  %[Operational Correspondence, Soundness, ${\tm{\cpgvC{\cdot}}}$]%
  If $\pcp{\seq{P}{\ty{\Gamma}}}$ and $\pgv{\tm{\cpgvC{P}}\cred\tm{\conf{C}}}$, there exists a $\tm{Q}$ such that $\pcp{\tm{P}\red^+\tm{Q}}$ and $\pgv{\tm{\conf{C}}\cred^\star\tm{\cpgvC{Q}}}$
\end{thm}
\begin{thm}\label{thm:pcp-to-pgv-operational-correspondence-completeness}
  %[Operational Correspondence, Completeness, ${\tm{\cpgvC{\cdot}}}$]%
  If $\pcp{\seq{P}{\ty{\Gamma}}}$ and $\pcp{\tm{P}\red\tm{Q}}$,
  then $\pgv{\tm{\cpgvC{P}}\cred^+\tm{\cpgvC{Q}}}$.
\end{thm}
\endgroup

